Extracting COVID-19 Diagnoses and Symptoms From Clinical Text: A New Annotated Corpus and Neural Event Extraction Framework

Coronavirus disease 2019 (COVID-19) is a global pandemic. Although much has been learned about the novel coronavirus since its emergence, there are many open questions related to tracking its spread, describing symptomology, predicting the severity of infection, and forecasting healthcare utilization. Free-text clinical notes contain critical information for resolving these questions. Data-driven, automatic information extraction models are needed to use this text-encoded information in large-scale studies. This work presents a new clinical corpus, referred to as the COVID-19 Annotated Clinical Text (CACT) Corpus, which comprises 1,472 notes with detailed annotations characterizing COVID-19 diagnoses, testing, and clinical presentation. We introduce a span-based event extraction model that jointly extracts all annotated phenomena, achieving high performance in identifying COVID-19 and symptom events with associated assertion values (0.83-0.97 F1 for events and 0.73-0.79 F1 for assertions). In a secondary use application, we explored the prediction of COVID-19 test results using structured patient data (e.g. vital signs and laboratory results) and automatically extracted symptom information. The automatically extracted symptoms improve prediction performance, beyond structured data alone.

==> tables/covid_auc.tex <==

%\begin{tabular}{lllll}
%\textbf{Note type}  & \textbf{\# Negative tests}    & \textbf{\# Positive tests}    & %\textbf{Features}     & \textbf{AUC}  \\ \toprule
%\multirow{3}{*}{ED} & \multirow{3}{*}{2,085}        & \multirow{3}{*}{142}          & structured            &               \\ \cmidrule{4-5}
%                    &                               &                               & notes                 &               \\ \cmidrule{4-5}
%                    &                               &                               & structured+notes      &               \\ \midrule
%Progress            & 5,982                         & 302                           & notes                 &               \\ \midrule
%Telephone           & 3,805                         & 248                           & %notes                 &               \\ \bottomrule
%\end{tabular}


%\newcolumntype{A}{ >{\raggedleft\arraybackslash} m{0.40in} }
\newcolumntype{A}{ >{\centering\arraybackslash} m{0.55in} }
\newcolumntype{B}{ >{\centering\arraybackslash} m{0.15in} }
\newcolumntype{C}{ >{\centering\arraybackslash} m{0.5in} }
\newcolumntype{D}{ >{\centering\arraybackslash} m{0.5in} }
\newcolumntype{E}{ >{\centering\arraybackslash} m{0.5in} }


\begin{tabular}{m{0.65in} A A B C D E}
%\begin{tabular}{m{0.72in} m{0.40in} m{0.40in} m{0.70in} m{0.40in} m{0.70in}}
\toprule
\multirow{3}{*}{\textbf{Note type}} & \multicolumn{2}{c}{\textbf{Gold tests}}               &   & \multicolumn{3}{c}{\textbf{AUC}}                 \\ \cmidrule{2-7}
                                    & \multirow{2}{*}{\textbf{\# negative}}         & \multirow{2}{*}{\textbf{\# positive}}   &   & \multirow{2}{*}{\textbf{structured}}       & \multirow{2}{*}{\textbf{notes}}    & \multirow{1}{0.5in}{\textbf{structured +notes}} \\
                                    &                                               &                        &   &                           &                   &                                   \\ \toprule
ED                                  & 2,085                        & 142                    &   & 0.73                      & 0.68              & 0.78$^*$                         \\
Progress                            & 5,982                        & 302                    &   & 0.63                      & 0.67              & 0.68$^*$                          \\
Telephone                           & 3,805                        & 248                    &   & 0.60                      & 0.65              & 0.66$^*$                          \\ \bottomrule                         
\end{tabular}


==> tables/extraction_performance_OUTDATED.tex <==

\newcolumntype{A}{ >{\raggedleft\arraybackslash} m{0.38in} }
\newcolumntype{B}{ >{\raggedleft\arraybackslash} m{0.65in} }
\newcolumntype{R}{ >{\raggedleft\arraybackslash} m{0.18in} }

%\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|}
\begin{tabular}{m{0.72in} m{0.71in} A R R R B R R R}
\toprule
\multirow{2}{*}{\textbf{Event type}} & \multirow{2}{*}{\textbf{Argument}} & \multicolumn{4}{c}{\textbf{Train-CV}}                   & \multicolumn{4}{c}{\hspace{0.27in}\textbf{Test}}                       \\ \cmidrule{3-10} 
                                     &                                    & \textbf{\# Gold} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{\# Gold} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \toprule
\multirow{3}{*}{COVID}               & Trigger                            &    3,931 & 0.95 & 0.97 & 0.96 & 1,497 & 0.96 & 0.97 & 0.97 \\         \cmidrule{2-10}                                                   
                                     & Assertion                          &    2,936 & 0.70 & 0.74 & 0.72 & 1,075 & 0.72 & 0.74 & 0.73 \\         
                                     & Test Status                        &     1,068 & 0.60 & 0.61 & 0.61 &   457 & 0.63 & 0.60 & 0.62 \\        \midrule                                                         
\multirow{8}{*}{Symptom}        & Trigger                            & 13,823 & 0.81 & 0.86 & 0.83 & 5,789 & 0.81 & 0.85 & 0.83 \\             \cmidrule{2-10}                                                 
                                     & Assertion                          &   13,833 & 0.76 & 0.80 & 0.78 & 5,791 & 0.77 & 0.80 & 0.79 \\         
                                     & Change                             &   739 & 0.54 & 0.05 & 0.09 &   341 & 0.45 & 0.05 & 0.09 \\            
                                     & Severity                           &     743 & 0.46 & 0.32 & 0.38 &   327 & 0.45 & 0.31 & 0.37 \\          \cmidrule{2-10}                                                   
                                     & Anatomy                            &  3,839 & 0.73 & 0.55 & 0.63 & 1,959 & 0.77 & 0.49 & 0.60 \\           
                                     & Characteristics                    &    3,145 & 0.56 & 0.26 & 0.36 & 1,441 & 0.66 & 0.25 & 0.36 \\         
                                     & Duration                           &   3,744 & 0.60 & 0.45 & 0.52 & 1,344 & 0.54 & 0.55 & 0.55 \\          
                                     & Frequency                          &      801 & 0.68 & 0.41 & 0.51 &   250 & 0.60 & 0.51 & 0.55 \\         \bottomrule                                    
\end{tabular}

==> tables/symptom_frequency_ed.tex <==





\begin{tabular}{llll}
\toprule
\textbf{Symptom}             & \textbf{March} & \textbf{April} &\textbf{ May}  \\ \midrule
cough               & 79\%  & 49\%  & 22\% \\
fever               & 57\%  & 34\%  & 12\% \\
shortness of breath & 52\%  & 34\%  & 20\% \\ \bottomrule
\end{tabular}

==> tables/symptom_normalization_w_quotes.tex <==


{\small


\renewcommand*{\arraystretch}{0.9}
\begin{longtable}{ p{1.2in} p{4.2in}}
\caption{Expert-derived mapping of symptoms to canonical forms} \\
\label{symptom_normalization} \\
%\input{tables/symptom_normalization.tex}
\toprule
\multicolumn{1}{l}{\textbf{Normalized symptom}}   & \multicolumn{1}{l}{\textbf{Symptom variants}} \\ \toprule \endfirsthead


\multicolumn{2}{l}{Table \ref{symptom_normalization} - continued from previous page}\\
\hline \multicolumn{1}{l}{\textbf{Normalized symptom}} & \multicolumn{1}{l}{\textbf{Symptom variants}} \\ \toprule
\endhead


\hline \multicolumn{2}{r}{{Continued on next page}} \\ \bottomrule
\endfoot

\bottomrule
\endlastfoot



``altered mental status''	&	``ams,'' ``confused,'' ``confusion''	\\ \midrule
``anxiety''	&	``agitated,'' ``agitation,'' ``anxious''	\\ \midrule
``arthralgia''	&	``arthralgias''	\\ \midrule
``bleeding''	&	``bleed,'' ``blood,'' ``bloody''	\\ \midrule
``bruising''	&	``bruise,'' ``bruises,'' ``ecchymosis''	\\ \midrule
``chest pain''	&	``cp''	\\ \midrule
``chills''	&	``chill''	\\ \midrule
``cough''	&	``c,'' ``c.,'' ``cough cough,'' ``coughing,'' ``coughs,'' ``distress coughing,'' ``distressed coughing''	\\ \midrule
``cramping''	&	``cramps''	\\ \midrule
``decreased appetite''	&	``loss of appetite,'' ``poor appetite,'' ``poor p.o. intake,'' ``poor po intake,'' ``reduced appetite''	\\ \midrule
``deformities''	&	``deformity''	\\ \midrule
``dehydration''	&	``dehydrated''	\\ \midrule
``diarrhea''	&	``d,'' ``d.,'' ``diarrhea stools,'' ``loose stools''	\\ \midrule
``disharge''	&	``drainage''	\\ \midrule
``distended''	&	``distention''	\\ \midrule
``dysphagia''	&	``difficulty swallowing,'' ``dysphagia symptoms''	\\ \midrule
``erythema''	&	``erythematous,'' ``redness''	\\ \midrule
``exudates''	&	``exudate''	\\ \midrule
``fall''	&	``falls''	\\ \midrule
``fatigue''	&	``drowsiness,'' ``drowsy,'' ``fatigued,'' ``somnolence,'' ``somnolent,'' ``tired,'' ``tiredness''	\\ \midrule
``fever''	&	``f,'' ``f.,'' ``febrile,'' ``fevers''	\\ \midrule
``flu-like symptoms''	&	``flu - like symptoms,'' ``influenza - like symptoms''	\\ \midrule
``gi symptoms''	&	``abdominal symptoms''	\\ \midrule
``headache''	&	``ha,'' ``headaches''	\\ \midrule
``heartburn''	&	``gerd symptoms,'' ``heartburn symptoms''	\\ \midrule
``hematochezia''	&	``brbpr''	\\ \midrule
``ill''	&	``ill - appearing,'' ``ill appearing,'' ``ill symptoms,'' ``illness,'' ``sick''	\\ \midrule
``incontinent''	&	``incontinence''	\\ \midrule
``irritation''	&	``irritable''	\\ \midrule
``itching''	&	``itchy''	\\ \midrule
``lethargy''	&	``lethargic''	\\ \midrule
``lightheadedness''	&	``dizziness,'' ``dizzy,'' ``headedness,'' ``lightheaded''	\\ \midrule
``myalgia''	&	``ache,'' ``aches,'' ``aching,'' ``bodyaches,'' ``myalgias''	\\ \midrule
``nausea''	&	``n,'' ``n.,'' ``nauseated,'' ``nauseous''	\\ \midrule
``pain''	&	``discomfort,'' ``painful,'' ``pains''	\\ \midrule
``pruritus''	&	``pruritis''	\\ \midrule
``rash''	&	``rashes''	\\ \midrule
``respiratory symptoms''	&	``uri symptoms''	\\ \midrule
``runny nose''	&	``rhinorrhea''	\\ \midrule
``seizures''	&	``seizure,'' ``seizures''	\\ \midrule
``shortness of breath''	&	``\_\_\_shortness of breath,'' ``difficult breathing,'' ``difficulty breathing,'' ``difficulty of breathing,'' ``distress breathing,'' ``distressed breathing,'' ``doe,'' ``dsypnea,'' ``dypsnea,'' ``dyspnea,'' ``dyspnea exertion,'' ``dyspnea on exertion,'' ``increase work of breathing,'' ``increased work of breathing,'' ``out of breath,'' ``respiratory distress,'' ``short of breath,'' ``shortneses of breath,'' ``shortness breath,'' ``shortness of breaths,'' ``sob,'' ``sob on exertion,'' ``trouble breathing,'' ``work of breathing''	\\ \midrule
``sore throat''	&	``pharyngitis''	\\ \midrule
``soreness''	&	``sore''	\\ \midrule
``sputum''	&	``sputum production''	\\ \midrule
``sweats''	&	``diaphoresis,'' ``nightsweats,'' ``sweating''	\\ \midrule
``swelling''	&	``edema,'' ``oedema,'' ``swollen''	\\ \midrule
``syncope''	&	``fainting''	\\ \midrule
``tenderness''	&	``tender''	\\ \midrule
``tremors''	&	``tremor''	\\ \midrule
``ulcers''	&	``ulcer,'' ``ulceration,'' ``ulcerations''	\\ \midrule
``urinary symptoms''	&	``urinary''	\\ \midrule
``urination''	&	``urinating''	\\ \midrule
``vomiting''	&	``emesis,'' ``v,'' ``v.,'' ``vomitting''	\\ \midrule
``weakness''	&	``weak''	\\ \midrule
``wheezing''	&	``wheeze,'' ``wheezes''	\\ \midrule
``wounds''	&	``wound''	\\ \bottomrule


\end{longtable}
}










%\begin{tabular}{m{1.3in} m{4.0in}}
%\hline \multicolumn{1}{|c|}{\textbf{First column}} & \multicolumn{1}{c|}{\textbf{Second column}} & \multicolumn{1}{c|}{\textbf{Third column}} \\ \hline 
%\endfirsthead
%\toprule


%\end{tabular}

==> tables/umls_extraction_performanceFULL.tex <==

\newcolumntype{A}{ >{\raggedleft\arraybackslash} m{0.38in} }
\newcolumntype{B}{ >{\raggedleft\arraybackslash} m{0.65in} }
\newcolumntype{R}{ >{\raggedleft\arraybackslash} m{0.18in} }

%\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|}
\begin{tabular}{m{1.1in} m{0.7in} A R R B R R}
\toprule

%\multicolumn{4}{c}{\hspace{0.27in}\textbf{Test}} 
%\begin{tabular}{llllllll}


\multirow{2}{*}{\textbf{Case}}              & \multirow{2}{*}{\textbf{Argument}}  & \multicolumn{3}{c}{\textbf{All semantic types}}     & \multicolumn{3}{c}{\hspace{0.27in}\textbf{``Sign or Symptom''}} \\ \cmidrule{3-8}
                                            &                                     & \textbf{P}  & \textbf{R}  & \textbf{F1}             & \textbf{P}  & \textbf{R}     & \textbf{F1}            \\  \toprule
\multirow{2}{*}{Exact trigger match}        & Trigger                             & 0.02        & 0.70        & 0.05                    & 0.53           & 0.54          & 0.54                 \\  
                                            & Assertion                           & 0.02        & 0.57        & 0.04                    & 0.43           & 0.44          & 0.44                 \\ \midrule
\multirow{2}{*}{Any triggers overlap}       & Trigger                             & 0.03        & \textbf{0.90}        & 0.06                    & \textbf{0.66}           & 0.67          & \textbf{0.66}                 \\
                                            & Assertion                           & 0.03        & \textbf{0.74}        & 0.05                    & \textbf{0.54}           & 0.55          & \textbf{0.54}                 \\ \bottomrule           
\end{tabular}
